Best-Arm Identification in Correlated Multi-Armed Bandits

In this paper we consider the problem of best-arm identification in multi-armed bandits in the fixed confidence setting, where the goal is to identify, with probability $1-\delta$ for some $\delta>0$, the arm with the highest mean reward in minimum possible samples from the set of arms $\mathcal{K}$. Most existing best-arm identification algorithms and analyses operate under the assumption that the rewards corresponding to different arms are independent of each other. We propose a novel correlated bandit framework that captures domain knowledge about correlation between arms in the form of upper bounds on expected conditional reward of an arm, given a reward realization from another arm. Our proposed algorithm C-LUCB, which generalizes the LUCB algorithm utilizes this partial knowledge of correlations to sharply reduce the sample complexity of best-arm identification. More interestingly, we show that the total samples obtained by C-LUCB are of the form $\mathcal{O}\left(\sum_{k \in \mathcal{C}} \log\left(\frac{1}{\delta}\right)\right)$ as opposed to the typical $\mathcal{O}\left(\sum_{k \in \mathcal{K}} \log\left(\frac{1}{\delta}\right)\right)$ samples required in the independent reward setting. The improvement comes, as the $\mathcal{O}(\log(1/\delta))$ term is summed only for the set of competitive arms $\mathcal{C}$, which is a subset of the original set of arms $\mathcal{K}$. The size of the set $\mathcal{C}$, depending on the problem setting, can be as small as $2$, and hence using C-LUCB in the correlated bandits setting can lead to significant performance improvements. Our theoretical findings are supported by experiments on the Movielens and Goodreads recommendation datasets.

==> spillover.tex <==
\begin{table}[t]
\parbox{.9\linewidth}{
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Algorithm} & \textbf{Sampling Strategy} & \textbf{Eliminate Arm $k$ from $\mathcal{A}_t$ if} &\textbf{Stopping Criteria}\\ \hline
Racing & Round Robin in $\mathcal{A}_t$                   &    $U_k\left(\frac{\delta}{K}\right) < \max_{\ell \in \mathcal{A}_t} L_\ell\left(\frac{\delta}{K}\right)$   & $|\mathcal{A}_t| = 1$             \\ \hline
lil'UCB & $k_{t} = \argmax_{k} U_k( \delta)$                   & $-$ & $n_{k_t} \geq \alpha \sum_{k \neq k_t} n_k$                 \\ \hline
LUCB & Sample $m_1, m_2$,~ $m_1 = \argmax_{k \in \mathcal{A}_t} \hat{\mu}_k$,                    & $U_k\left(\frac{\delta}{K}\right) < \max_{\ell \in \mathcal{A}_t} L_\ell\left(\frac{\delta}{K}\right)$*  &    $|\mathcal{A}_t| = 1$* or              \\ 
 &       $m_2 = \argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} U_k\left(\frac{\delta}{K}\right)$   &   & $L_{m_1}\left(\frac{\delta}{K}\right) > U_{m_2}\left(\frac{\delta}{K}\right)$                 \\ \hline
LUCB++ & Sample $m_1, m_2$,~ $m_1 = \argmax_{k \in \mathcal{K}} \hat{\mu}_k$,                    &  \quad -  &  $L_{m_1}\left(\frac{\delta}{2K}\right) > U_{m_2}\left(\frac{\delta}{2}\right)$            \\ 
 &       $m_2 = \argmax_{k \in \mathcal{K} \setminus \{ {m_1}\}} U_k\left(\frac{\delta}{2}\right)$   &   &                  \\ \hline
 \textbf{C-LUCB} & Sample $m_1, m_2$,~ $m_1 = \argmax_{k \in \mathcal{A}_t} I_k(t)$,                    & $\tilde{U}_k\left( \frac{2\delta}{3K}\right) < \max_{\ell \in \mathcal{A}_t} L_\ell\left( \frac{2\delta}{3K}\right)$  &    $|\mathcal{A}_t| = 1$               \\ 
\textbf{(ours)}  &    $m_2 = \argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} \min\left(\tilde{U}_{k,k}\left(\frac{2\delta}{3K}\right), I_k(t)\right)$   &   &                  \\ \hline
\textbf{C-LUCB++} & Sample $m_1, m_2$,~ $m_1 = \argmax_{k \in \mathcal{A}_t} I_k(t)$,                    &  $\tilde{U}_k\left( \frac{\delta}{3K}\right) < \max_{\ell \in \mathcal{A}_t} L_\ell\left( \frac{\delta}{3K}\right)$  &  $|\mathcal{A}_t| = 1$ or          \\ 
 \textbf{(ours)} &       $m_2 = \argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} \min\left(\tilde{U}_{k,k}\left(\frac{\delta}{2}\right), I_k(t)\right)$   &   &  $L_{m_1}\left(\frac{\delta}{4K}\right) > \tilde{U}_{m_2, m_2}\left(\frac{\delta}{4}\right)$                \\ \hline 
\end{tabular}
}
\caption{All best-arm identification algorithms have three key components, i) Sampling strategy at each round $t$, ii) elimination criteria for an arm and iii) the stopping criteria of the algorithm. We compare these for Racing, lil'UCB, LUCB and LUCB++ algorithms and see the differences in their operation.}
\GJ{This table shouldn't spill into the margin. You could break some of the long equations into two lines to save horizontal space}
\SG{Put correct caption referencing the indices $I_k$ and $\tilde{U}_k$}
\SG{I am unsure on how to write the caption here, as it contains the content of our algorithms as well}
\label{tab:summaryAlgoClassic}
\vspace{-0.2cm}
\end{table}


\begin{table}[t]
\parbox{.9\linewidth}{
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Algorithm} & \textbf{$m_1(t)$} & \textbf{$m_2(t)$} &\textbf{$1 - \delta$ guarantee?} & \textbf{Theorem 2?} & \textbf{Samples}\\ \hline
\textbf{C-LUCB} &  $\argmax_{k \in \mathcal{A}_t} I_k(t)$   & $\argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} \min\left(\tilde{U}_{k,k}\left(\frac{2\delta}{3K}\right), I_k(t)\right)$ & Yes   &  Yes  &  TBA        \\ \hline
\textbf{maxmin-LUCB} & $\argmax_{k \in \mathcal{A}_t} \min_{\ell} \hat{\phi}_{k,\ell}(t)$   & $\argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} \tilde{U}_k\left(\frac{2\delta}{3K}\right)$ & Yes   &  ?  &  TBA        \\ \hline
\textbf{2-LUCB} & $\argmax_{k \in \mathcal{A}_t} I_k(t)$   & $\argmax_{k \in \mathcal{A}_t \setminus \{ {m_1}\}} \tilde{U}_k\left(\frac{2\delta}{3K}\right)$ & Yes   &  ?  &  TBA        \\ \hline 

\end{tabular}
}
\caption{Potential variants of the C-LUCB algorithm.\SG{Split this table to fit in the paper}}
\label{tab:variantsCLUCB}
\vspace{-0.2cm}
\end{table}

\subsection{Variants of C-LUCB}

\begin{proof}
\SG{Clean this proof}
 Suppose that algorithm samples arm $k \neq k^*$ at round $t$. We will show that in such a situation, the stopping criteria can not be satisfied and hence algorithm will not stop after sampling a sub-optimal arm $k \neq k^*$. 

Define $\mathcal{E}_1$ to be the event that empirical mean of all arm lie within their confidence intervals uniformly for all $t \geq 1$
\begin{equation}
\Bigg\{ \forall{t \geq 1, k \in \mathcal{K}}, ~~~ \hat{\mu}_k(t) - C_{n_k}\left(\frac{2\delta}{3K}\right) \leq \mu_k \leq \hat{\mu}_k + C_{n_k}\left(\frac{2\delta}{3K}\right) \Bigg\}    
\label{assump:wellBehaved}
\end{equation} 

Define $\mathcal{E}_2$ to be the event that empirical pseudo-reward of optimal arm with respect to all other arms lie within their confidence intervals uniformly for all $t \geq 1$, i.e., 
\begin{equation}
\Bigg\{ \forall{t \geq 1, \ell \in \mathcal{K}}, ~~~ \phi_{k^*,\ell} \leq \hat{\phi}_{k^*,\ell}(t) + C_{n_\ell}\left(\frac{2\delta}{3K}\right) \Bigg\}    
\label{assump:PseudowellBehaved}
\end{equation} 
Define $\mathcal{E} = \mathcal{E}_1 \cap \mathcal{E}_2$. See that $\Pr(\mathcal{E}) \geq 1 - \delta$. See Lemma z. 

[This happens because of the construction of LIL bounds and their property \Cref{eqn:MainAssumption}.]

When can the algorithm stop with arm $k \neq k^*$?\\
It only happens if arm $k$ is sampled in round $t+1$, and one of the two things listed below happens if Arm $k$ is the only arm in set $\mathcal{A}_t$. In such a scenario, $\exists \tau, k \neq k^*: U_{k^*}(\tau) < L_k(\tau)$. This can only occur if one of the following events occur, 
\begin{enumerate}
    \item $U_{k^*,k^*}(\tau) < L_k(\tau)$
    \item $U_{k^*,\ell}(\tau) < L_k(\tau) \quad \ell \neq k^*$
\end{enumerate}

See that under the event $\mathcal{E}$, $U_{k^*,\ell}(\tau) > \mu_{k^*}$ and $L_k(\tau) < \mu_k \quad \forall{\tau,k}$. This shows that under the event $\mathcal{E}$, $U_{k^*}(\tau) > L_k(\tau) \quad \forall{k, \tau}$ as $\mu_{k^*} > \mu_{k} \quad \forall{k \neq k^*}$. This implies that the algorithm returns the best arm with probability at least $1 - \delta$ as $\Pr(\mathcal{E}^{c}) \leq \delta$.
\end{proof}



\begin{algorithm}[t]
\hrule 
\vspace{0.1in}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Confidence $\delta$, $1-\delta$ Confidence bound $C(., \delta)$.
\STATE \textbf{Initialize:} $\pulls_\arm = 0, U_\arm = \infty, L_k = - \infty$,  for all $\arm \in \{1, 2, \dots \numArms\}$
\STATE Play each arm once
\STATE \textbf{Maintain:} $U_k\left(n_k, \frac{\delta}{K}\right) = \hat{\mu}_k + C\left(n_k, \frac{\delta}{K}\right), L_k\left(n_k, \frac{\delta}{K}\right) = \hat{\mu}_k - C\left(n_k, \frac{\delta}{K}\right) \quad \forall{k \in \mathcal{K}}$
\FOR{ each round $\slot$}
\STATE $h_t = \argmax_{k \in \mathcal{K}} \hat{\mu}_k(t)$
\STATE $l_t = \argmax_{k \neq h_t} U_k\left(n_k, \frac{\delta}{K}\right)$
\IF{$L_{h_t}\left(n_{h_t}, \frac{\delta}{K}\right) > U_{l_t}\left(n_{l_t}, \frac{\delta}{K}\right)$}
\STATE Stop and declare $h_t$ as the best-arm
\ELSE
\STATE Play arm $h_t, l_t$ and observe rewards
\ENDIF
\STATE Update empirical rewards $\hat{\mu}_{h_t}(t), \hat{\mu}_{l_t}(t)$, UCB indices $U_{h_t}\left(n_{h_t}, \frac{\delta}{K}\right), U_{l_t}\left(n_{h_t} \frac{\delta}{K}\right)$ and LCB indices $L_{h_t}\left(n_{l_t}, \frac{\delta}{K}\right), L_{l_t}\left(n_{l_t},\frac{\delta}{K}\right)$. 
\ENDFOR
\end{algorithmic}
\vspace{0.1in}
\hrule
\caption{LUCB Algorithm}
\label{alg:formalAlgo}
\vspace{-0.2cm}
\end{algorithm}







\begin{algorithm}[t]
\hrule 
\vspace{0.1in}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Confidence $\delta$, $1-\delta$ Confidence bound $C(., \delta)$.
\STATE \textbf{Initialize:} $\pulls_\arm = 0, U_\arm = \infty, L_k = - \infty$,  for all $\arm \in \{1, 2, \dots \numArms\}$, Set of Active arms $\mathcal{A}(0) = \mathcal{K}$
\STATE Play each arm once
\STATE \textbf{Maintain:} $U_{k,\ell}\left(n_\ell, \frac{\delta}{K}\right) = \hat{\phi}_{k,\ell} + C\left(n_\ell, \frac{\delta}{K}\right), ~~ U_k\left(\frac{\delta}{K}\right) = \min_{\ell \in \mathcal{K}} U_{k,\ell}\left(n_\ell, \frac{\delta}{K}\right)$
\STATE $L_k\left(n_k, \frac{\delta}{K}\right) = \hat{\mu}_k - C\left(n_k, \frac{\delta}{K}\right) $
\STATE $I_{k,\ell}(t) = \hat{\phi}_{k, \ell}(t) + B\sqrt{\frac{2 \log t}{n_{\ell}(t)}}, ~~ I_k(t) = \min_{\ell \in \mathcal{K}} I_{k, \ell}(t)$
\FOR{ each round $\slot$}
\IF{$|\mathcal{A}_t| = 1$}
\STATE Stop and declare the single arm in $\mathcal{A}_t$ as the best-arm
\ENDIF
\STATE $h_t = \argmax_{k \in \mathcal{A}_t} I_k(t)$
\STATE $l_t = \argmax_{k \neq \mathcal{A}_t \setminus \{h_t\}} \min \left(U_{k,k}\left(n_k, \frac{\delta}{K}\right), I_k(t) \right)$
\STATE Play arms $h_t, l_t$
\STATE \textbf{Eliminate Arms:} 
\IF{$U_k\left(\frac{\delta}{K}\right) < \max_{k \in \mathcal{K}} L_k\left(\frac{\delta}{K}\right)$}
\STATE $\mathcal{A}_t = \mathcal{A}_t \setminus \{k\}$
\ENDIF
\STATE Update  UCB indices $U_{k}\left(n_{k}, \frac{\delta}{K}\right)$, LCB indices $L_{k}\left(n_{k}, \frac{\delta}{K}\right),$ and Regular indices $I_k(t) \quad \forall{k \in \mathcal{K}}$. 
\ENDFOR
\end{algorithmic}
\vspace{0.1in}
\hrule
\caption{C-LUCB Algorithm}
\label{alg:formalAlgo}
\vspace{-0.2cm}
\end{algorithm}
